Electrodynamics and dissipation in the binary magnetosphere of pre-merger neutron stars

We investigate energy release in the interacting magnetospheres of binary neutron stars (BNSs) with global 3D force-free electrodynamics simulations. The system dynamics depend on the inclinations $\chi_1$ and $\chi_2$ of the stars' magnetic dipole moments relative to their orbital angular momentum. The simplest aligned configuration ($\chi_1=\chi_2=0^\circ$) has no magnetic field lines connecting the two stars. Remarkably, it still develops separatrix current sheets warping around each star and a dissipative region at the interface of the two magnetospheres. A Kelvin-Helmholtz (KH)-type instability drives significant dissipation at the magnetospheric interface, generating local Alfv\'enic turbulence and escaping fast magnetosonic waves. Binaries with inclined magnetospheres release energy in two ways: via KH instability at the interface and via magnetic reconnection flares in the twisted flux bundles connecting the companions. Outgoing compressive waves occur in a broad range of BNS parameters, possibly developing shocks and sourcing fast radio bursts. We discuss implications for X-ray and radio precursors of BNS mergers.

==> referee.tex <==
The manuscript "Electrodynamics and dissipation in the binary magnetosphere of pre-merger neutron stars" by Jens Malhmann and Andrei Belobodorov presents new results from force-free electrodynamics simulations of binary neutron star magnetospheres. The authors show a new mechanism of magnetospheric energy dissipation previously overlooked in global simulations: Kelvin Helmholtz instability (KHI) in the interface of the two magnetospheres. The instability drives turbulence and fast magnetosonic waves that dissipate energy even in the case where the magnetic dipole of the stars is aligned with the orbital momentum. The authors also explore the effects of different inclinations on the instability and on the outgoing Poynting flux.

The results are interesting, sufficiently novel, and carefully justified. The appendix includes analytical and local simulations that support the conclusions from the global 3D simulations in the paper. Although the numerical techniques here are not new, and similar simulations were performed in the past, it is, as far as I know, the first time that the magnetospheric KHI is explicitly shown in a global simulation. Some of the consequences of this instability can only be speculated about given the limitation of the force-free setup; however, this opens the door to further investigations.

I am happy to recommend this paper for publication in ApJ Letters after some minor clarifications I outline below.

########################### Author reply:
We thank the referee for their thorough review of our work and for bringing forward several thoughtful suggestions to improve our manuscript. Our detailed responses are below, and changes in the paper are marked in red color.
#########################################

Line 21: The paper is generally well written but the abstract could be much better structured in my opinion. For instance, in this line, it sounds like the outgoing compressive waves are generated only in the inclined case, which is not the case, right?

########################### Author reply:
We have slightly improved the abstract. The outgoing waves are generated in all cases, however, they have the best chance to steepen into shocks in inclined geometries. 
#########################################

Line 56: The authors might consider referencing previous simulations exploring force-free magnetospheres of binary neutron stars such as Carrasco & Shibata 2020 and Palenzuela et al 2013.

########################### Author reply:
We included the suggested references in our introduction section (lines 55 and 65). 
#########################################

Line 90: I agree the main conclusion about the dissipation mechanism is most likely not affected by non-inertial effects but wouldn't it affect wave propagation?

########################### Author reply:
We have added a sentence highlighting the possible role of non-inertial effects on wave propagation in line 492. We do not anticipate a significant alteration of FMS wave propagation properties due to orbital motion for short-wavelength signals. However, the presence of electric fields due to the orbital motion can alter the relative strength of the electric field E/B. This may mildly affect the dissipation of strong FMS waves or if and where they become non-linear.
#########################################

Line 94: Might be useful to clarify the motivation behind the choice of Omega_*. Shouldn't it be -2Omega_Keplerian for an irrotational binary in the corotating frame?

########################### Author reply:
Yes, our choice of Omega_* approximately corresponds to the Keplerian frequency Omega. When both stars have zero angular momenta in the lab frame (no tidal locking), they are spinning with -Omega in the frame that co-rorates with the orbital motion. We have clarified this choice in footnote 1.
#########################################

Line 173: The explanation is convincing but I feel the authors could show a 2D snapshot of field lines as in Figure 1 (lower panel) but of the actual simulation to observe this more clearly.

########################### Author reply:
We would like to keep the simpler version of Figure 1 for two reasons: (1) it illustrates our initial conditions (apart from indicating schematically the anticipated dissipation sites) and (2) a snapshot of the simulation in the xz plane would anyway not show the most interesting (and very different) cross sections where rotation compresses the magnetosphere. 
#########################################

Line 240: If there were no dissipation in the interface, I gather that the Poynting flux measured at larger radii would be larger. Although this region acts as an energy sink in this FFE setup, how much of the energy is carried by the FMS?

########################### Author reply:
For aligned companions, our analysis identifies an upper limit of 5\% if the Poynting flux is carried by FMS waves. This is mentioned in the paper.
#########################################

If non-ideal effects were included, do the authors expect changes in how the perturbations occur and propagate from the KHI interface?

########################### Author reply:
We do not expect non-ideal effects to dramatically change the generated waves -- they are generated by the twists and compressions in KHI, which should be reasonably well captured by FFE. We think waves can be changed more significantly by MHD inertia effects (local drop in sigma in response to dissipation). The need of future MHD simulations is mentioned in the end of the paper. 
#########################################

Are the authors able to simulate the non-linear phase of the FFE KHI in their local box simulation?

########################### Author reply:
We do not model the non-linear phase of the KH instability in our local simulations. The periodic box setup has a finite energy supply of the shear layer (it is not a driven system). The system rapidly relaxes to a steady state after the instability onset.
#########################################
